When Robotics Meets Wireless Communications: An Introductory Tutorial

The importance of ground Mobile Robots (MRs) and Unmanned Aerial Vehicles (UAVs) within the research community, industry, and society is growing fast. Many of these agents are nowadays equipped with communication systems that are, in some cases, essential to successfully achieve certain tasks. In this context, we have begun to witness the development of a new interdisciplinary research field at the intersection of robotics and communications. This research field has been boosted by the intention of integrating UAVs within the 5G and 6G communication networks. This research will undoubtedly lead to many important applications in the near future. Nevertheless, one of the main obstacles to the development of this research area is that most researchers address these problems by oversimplifying either the robotics or the communications aspect. This impedes the ability of reaching the full potential of this new interdisciplinary research area. In this tutorial, we present some of the modelling tools necessary to address problems involving both robotics and communication from an interdisciplinary perspective. As an illustrative example of such problems, we focus in this tutorial on the issue of communication-aware trajectory planning.

==> notes.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
-antenna issues ,antenna placement on the UAV, antenna orientation, add:
[60] C.-M. Cheng, P.-H. Hsiao, H. T. Kung, and D. Vlah, “Performance
measurement of 802.11a wireless links from UAV to ground nodes with
various antenna orientations,” in Proc. Int. Conf. Comput. Commun.
Netw. (ICCCN), Arlington, VA, USA, 2006, pp. 303–308.
[61] E. Yanmaz, R. Kuschnig, and C. Bettstetter, “Channel measurements over 802.11a-based UAV-to-ground links,” in Proc. IEEE Glob.
Commun. Conf. (GLOBECOM) Workshops, Houston, TX, USA, 2011,
pp. 1280–1284
[84] E. Yanmaz, R. Kuschnig, and C. Bettstetter, “Achieving air-ground
communications in 802.11 networks with three-dimensional aerial
mobility,” in Proc. IEEE INFOCOM, 2013, pp. 120–124.
[85] N. Ahmed, S. S. Kanhere, and S. Jha, “On the importance of link
characterization for aerial wireless sensor networks,” IEEE Commun.
Mag., vol. 54, no. 5, pp. 52–57, May 2016.
-frequencies? attenuation due to gases in milimiter frequencies
-control link, data link, telemetry
[106] J. Chen, D. Raye, W. Khawaja, P. Sinha, and I. Guvenc, “Impact of 3D
UWB antenna radiation pattern on air-to-ground drone connectivity,”
in Proc. Veh. Technol. Conf. (VTC), Chicago, IL, USA, Aug. 2018,
pp. 1–5.
[107] W. Khawaja, O. Ozdemir, F. Erden, I. Guvenc, and D. Matolak, “UWB
air-to-ground propagation channel measurements and modeling using
UAVs,” in Proc. IEEE Aerosp. Conf., 2019.
[108] W. Khawaja, O. Ozdemir, and I. Guvenc, “Temporal and spatial characteristics of mmWave propagation channels for UAVs,” in Proc. Glob.
Symp. Millimeter Waves (GSMM), Boulder, CO, USA, May 2018,
pp. 1–6.
[68] M. Simunek, F. P. Fontán, and P. Pechac, “The UAV low elevation
propagation channel in urban areas: Statistical analysis and timeseries generator,” IEEE Trans. Antennas Propag., vol. 61, no. 7,
pp. 3850–3858, Jul. 2013
[126] T. Tavares et al., “Generalized LUI propagation model for UAVs communications using terrestrial cellular networks,” in Proc. IEEE Veh.
Technol. Conf. (VTC), Boston, MA, USA, 2015, pp. 1–6

A-A channel
[94] M. Walter, S. Gligorevic, T. Detert, and M. Schnell, “UHF/VHF air- ´
to-air propagation measurements,” in Proc. IEEE Eur. Conf. Antennas
Propag. (EuCAP), Barcelona, Spain, 2010, pp. 1–5.
[95] N. Goddemeier and C. Wietfeld, “Investigation of air-to-air channel
characteristics and a UAV specific extension to the Rice model,” in
Proc. IEEE Glob. Commun. (Globecom) Workshops, San Diego, CA,
USA, Dec. 2015, pp. 1–5


